Quantum-Inspired Solver for Simulating Material Deformations

This paper explores the application of tensor networks (TNs) to the simulation of material deformations within the framework of linear elasticity. Material simulations are essential computational tools extensively used in both academic research and industrial applications. TNs, originally developed in quantum mechanics, have recently shown promise in solving partial differential equations (PDEs) due to their potential for exponential speedups over classical algorithms. Our study successfully employs TNs to solve linear elasticity equations with billions of degrees of freedom, achieving exponential reductions in both memory usage and computational time. These results demonstrate the practical viability of TNs as a powerful classical backend for executing quantum-inspired algorithms with significant efficiency gains. This work is based on our research conducted with IKERLAN.

==> images/drawings/trapezoid0.tex <==

\begin{tikzpicture}[scale=1.4]

% Define the number of rows and columns
\def\nrows{3}
\def\ncols{3}

% Define the transformation parameters
\def\ux{1}
\def\uy{0.1}
\def\vx{0.2}
\def\vy{0.8}
\def\wx{-0.1}
\def\wy{-0.06}

% Draw the deformed grid
\foreach \i in {0,...,\ncols} {
    \foreach \j in {0,...,\nrows} {
        % Calculate the deformed position
        \pgfmathsetmacro\x{\ux * \i + \vx * \j + \wx * \i * \j}
        \pgfmathsetmacro\y{\uy * \i + \vy * \j + \wy * \i * \j}
        
        % Draw the nodes
        \fill (\x, \y) circle (1.5pt);
        
        % Draw the horizontal lines
        \ifnum\i<\ncols
            \pgfmathsetmacro\nextx{\ux * (\i+1) + \vx * \j + \wx * (\i+1) * \j}
            \pgfmathsetmacro\nexty{\uy * (\i+1) + \vy * \j + \wy * (\i+1) * \j}
            \draw[thick] (\x, \y) -- (\nextx, \nexty);
        \fi
        
        % Draw the vertical lines
        \ifnum\j<\nrows
            \pgfmathsetmacro\nextx{\ux * \i + \vx * (\j+1) + \wx * \i * (\j+1)}
            \pgfmathsetmacro\nexty{\uy * \i + \vy * (\j+1) + \wy * \i * (\j+1)}
            \draw[thick] (\x, \y) -- (\nextx, \nexty);
        \fi
        
        % Draw nodes at the center of each square
        % \ifnum\i<\ncols
        %     \ifnum\j<\nrows
        %         \pgfmathsetmacro\centerx{\ux * (\i+0.5) + \vx * (\j+0.5) + \wx * (\i+0.5) * (\j+0.5)}
        %         \pgfmathsetmacro\centery{\uy * (\i+0.5) + \vy * (\j+0.5) + \wy * (\i+0.5) * (\j+0.5)}
        %         \fill[blue] (\centerx, \centery) circle (1pt);
        %     \fi
        % \fi
    }
}

% Draw the x and y axes
\draw[->,dashed] (-1, -.1) -> (5, .5) node[below,scale = 0.7] {$x$};
\draw[->,dashed] (-.2, -0.8) -> (1, 4) node[left, scale = 0.7] {$y$};

% Draw the x and y axes
\draw[->] (-1, 0) -> (5, 0) node[below,scale = 0.7] { $\eta$};
\draw[->] (0, -1) -> (0, 4) node[left, scale = 0.7] {$\xi$};

% Draw the nodes's labes
\node at (-.13, .13) {\small $0$};
\node at (.1, -.13) {\small $0$};
%\node at (3, .1) {\small $2^2 \smallminus 1$};
%\node at (.3, 2.7) {\small $2^2 \smallminus 1$};

\end{tikzpicture}


==> sections/PINNs.tex <==
\section{Physics Informed Neural Natworks}
\label{sec: PINNs}

\section{Introduction}
Physics-Informed Neural Networks (PINNs) represent a novel approach to integrating physical laws into the framework of neural networks. Traditional machine learning models often require extensive data for training and may not incorporate underlying physical principles governing the systems they are modeling. PINNs address this limitation by embedding physical laws, described by differential equations, into the training process, allowing the models to adhere to known behaviors and constraints of the system \citep{raissi2019physics}.

\section{Background}
The integration of physical principles into neural networks is not merely a novel experiment; it is a response to the critical need for models that can predict phenomena where data is scarce, expensive to obtain, or when the systems are governed by well-understood physical laws. The concept of PINNs is rooted in the idea that the laws of physics, which are typically expressed as differential equations, can be used as additional constraints during the training of neural networks. This approach enables the networks to learn not only from the data but also from the underlying physics of the problem, leading to more accurate and generalizable models \citep{karpatne2017theory}.

\section{Theoretical Framework}
A PINN is designed to solve problems described by partial differential equations (PDEs). Given a PDE of the form
\begin{equation}
    \mathcal{L}(u(x,t);\lambda) = 0,
\end{equation}
where $\mathcal{L}$ is a differential operator, $u(x,t)$ is the solution of the PDE, and $\lambda$ represents the parameters or coefficients within the PDE, the goal of a PINN is to approximate $u(x,t)$ by training a neural network \citep{raissi2019physics}.

The training process involves minimizing a loss function that is composed of two parts: a data mismatch term and a physics-informed term. The data mismatch term ensures that the neural network's predictions are consistent with the available observations, while the physics-informed term enforces the compliance of the network's outputs with the governing differential equations. Mathematically, the loss function can be expressed as
\begin{equation}
    \mathcal{L}_{total} = \mathcal{L}_{data} + \lambda_{p}\mathcal{L}_{physics},
\end{equation}
where $\mathcal{L}_{data}$ is the data mismatch loss, $\mathcal{L}_{physics}$ is the physics-informed loss, and $\lambda_{p}$ is a weighting factor that balances the two terms \citep{raissi2019physics}.

\section{Applications and Future Directions}
PINNs have found applications across a wide range of fields, including fluid dynamics, material science, and geophysics. By leveraging the power of PINNs, researchers can tackle complex problems such as simulating fluid flow around obstacles, predicting material properties under various conditions, and modeling seismic wave propagation. The future of PINNs lies in expanding their applicability, improving their efficiency, and integrating them with other machine learning approaches to solve multifaceted problems in science and engineering \citep{karniadakis2021physics}.


\section{Application of PINNs to Finite Element Problems in Linear Elasticity}

Finite Element Analysis (FEA) is a computational technique used extensively in engineering for solving problems in the field of linear elasticity, such as stress analysis in solid structures. However, traditional FEA methods require discretization of the domain into a mesh, which can be computationally expensive and time-consuming, especially for complex geometries or when dealing with dynamic boundary conditions. Physics-Informed Neural Networks (PINNs) present an alternative approach that can complement or, in some cases, substitute traditional FEA methods by leveraging the power of deep learning.

\subsection{The Linear Elasticity Problem}

Linear elasticity describes the behavior of solid materials under external forces, assuming small deformations and linear relationships between the stresses and strains in the material. The governing equations for a linear elasticity problem in an isotropic and homogeneous material can be expressed as the Navier-Lamé equations:
\begin{equation}
    -\mu \nabla^2 \mathbf{u} - (\lambda + \mu) \nabla(\nabla \cdot \mathbf{u}) = \mathbf{f},
\end{equation}
where $\mathbf{u}$ represents the displacement field within the material, $\mathbf{f}$ is the body force per unit volume acting on the material, and $\lambda$ and $\mu$ are Lamé's first and second parameters, respectively, which are material properties.

\subsection{PINNs Approach to Linear Elasticity}

The application of PINNs to linear elasticity involves training a neural network to approximate the displacement field $\mathbf{u}$ by minimizing a loss function that incorporates both the physical constraints, derived from the Navier-Lamé equations, and any available observational data. This physics-informed loss ensures that the predicted displacement field satisfies both the governing physical laws and the boundary conditions of the problem. Specifically, the physics-informed term of the loss function is formulated to penalize deviations from the Navier-Lamé equations across the domain of interest.

One of the key advantages of using PINNs for solving linear elasticity problems is their ability to handle complex boundary conditions and geometries without the need for mesh generation. This capability not only reduces the preprocessing time significantly but also enables the handling of problems where the geometry or boundary conditions change over time.

\subsection{Integration with Finite Element Methods}

While PINNs offer a powerful standalone tool for solving linear elasticity problems, they can also be integrated with traditional Finite Element methods to enhance their performance or to tackle specific challenges. For instance, PINNs can be used to generate solutions within each element of a finite element mesh, effectively serving as a mesh-free method for evaluating the displacements and stresses. Alternatively, PINNs can assist in optimizing the placement of elements or in refining the mesh based on the learned stress distribution, thereby improving the accuracy and efficiency of finite element simulations.

\subsection{Conclusion}

The application of Physics-Informed Neural Networks to Finite Element problems, especially in the context of linear elasticity, opens up new avenues for solving complex engineering problems. By embedding physical laws into the learning process, PINNs can provide accurate, efficient, and mesh-free solutions to problems that were traditionally addressed using Finite Element Analysis. This integration of machine learning with computational mechanics holds great promise for advancing the field of computational engineering and for developing innovative solutions to challenging problems in material science and structural engineering.



\section{Conclusion}
Physics-Informed Neural Networks offer a powerful tool for integrating physical laws into the fabric of machine learning models. By enforcing the adherence to known principles, PINNs provide a promising avenue for advancing the capabilities of neural networks in scientific computing and beyond. As research in this area continues to grow, the potential for groundbreaking applications and enhancements to existing methodologies seems limitless.




==> sections/introTN.tex <==
\section{Introduction to Tensor Networks}
\label{sec: Tensor Networks}

Tensor networks represent a powerful framework for expressing high-dimensional tensors in a decomposed format that significantly reduces the computational complexity associated with their storage and manipulation. Among the various tensor network formats, the tensor train (TT) decomposition stands out for its versatility and efficiency. This chapter delves into the mathematical formalism of tensor trains, introducing the tensor train decomposition for vectors, known as Matrix Product States (MPS), and for matrices, elaborating on their structure, decomposition process, and applications.

\subsection{Preliminaries}
Before proceeding to the tensor train decomposition, it is essential to understand the basic concepts underlying tensors and their operations. A tensor is a multidimensional array of numerical values, generalizing scalars, vectors, and matrices to higher dimensions. The \emph{order} of a tensor is the number of dimensions, also known as modes or ways.

\subsubsection{Tensor Operations}
Several operations are fundamental to tensor manipulations, including tensor product, tensor contraction, and tensor reshaping. These operations form the basis of tensor train decompositions and their applications.

\subsection{Tensor Train Decomposition}
The tensor train decomposition represents a tensor as a sequence of three-dimensional tensors (for vectors) or four-dimensional tensors (for matrices) in a train-like structure. The key advantage of this format is its ability to efficiently represent very high-dimensional tensors with a relatively low number of parameters.

\subsection{Tensor Train Decomposition for Vectors (MPS)}
Matrix Product States (MPS) are a particular case of tensor train decomposition applied to vectors. Given a vector $\mathbf{x} \in \mathbb{R}^{n_1 \times n_2 \times \cdots \times n_d}$, it can be decomposed as:

\begin{equation}
x_{i_1, i_2, \ldots, i_d} = G_1[i_1]G_2[i_2]\cdots G_d[i_d],
\end{equation}

where $G_k[i_k]$ represents a matrix for each index $i_k$ of the $k$-th dimension, except for the first and last matrices, which are vectors. This decomposition allows for a compact representation of the vector, exploiting its internal structure.

\subsubsection{Tensor Train Decomposition for Matrices}
The extension of MPS to matrices leads to a similar decomposition, where a matrix $\mathbf{A} \in \mathbb{R}^{(n_1 \times n_2 \times \cdots \times n_d) \times (m_1 \times m_2 \times \cdots \times m_d)}$ is represented in a tensor train format. The decomposition takes the form:

\begin{equation}
A_{(i_1, \ldots, i_d), (j_1, \ldots, j_d)} = G_1[i_1, j_1]G_2[i_2, j_2]\cdots G_d[i_d, j_d],
\end{equation}

where each $G_k[i_k, j_k]$ is a matrix, allowing the matrix $\mathbf{A}$ to be efficiently represented and manipulated.

\subsubsection{Bond Dimensions}
The bond dimension, denoted as $\chi$, is a critical parameter in the tensor train decomposition. It controls the size of the matrices or tensors at each position in the train, except for the first and last tensors, which are vectors. For a tensor train decomposed into $d$ tensors, the bond dimensions between these tensors can be denoted as $\chi_1, \chi_2, \ldots, \chi_{d-1}$, where each $\chi_i$ corresponds to the size of the bond between the $i$-th and $(i+1)$-th tensor in the train.

The choice of bond dimension has a significant impact on both the accuracy of the decomposition and the computational resources required for storage and operations. A higher bond dimension allows for a more accurate representation of the original tensor, at the cost of increased computational and storage requirements. Conversely, a lower bond dimension reduces the computational load and storage but may lead to a loss of information or accuracy.

\subsubsection{Effect of Bond Dimension on Representation}
\begin{itemize}
    \item \textbf{Accuracy vs. Complexity:} The bond dimension is the key to balancing the trade-off between the accuracy of the tensor representation and the computational and storage complexities. Optimal choice of bond dimensions, often through iterative algorithms or a priori estimates based on the tensor's properties, is crucial for efficient tensor train decompositions.
    \item \textbf{Expressive Power:} The bond dimensions determine the expressive power of the tensor train decomposition. With sufficient bond dimension, tensor trains can compactly represent exponentially large data with polynomial resources.
    \item \textbf{Adaptive Decomposition:} In practice, adaptive algorithms adjust the bond dimensions dynamically during the decomposition process to maintain a balance between approximation accuracy and resource constraints. This adaptability is essential for practical applications involving large-scale tensors.
\end{itemize}

\subsection{Basic Tensor Network Operations and Bond Dimension Dynamics}
Tensor train decompositions facilitate a variety of operations on tensors, including reshaping, slicing, and contracting, which are essential for manipulating and exploiting the structure of tensor networks. These operations have direct implications for the bond dimensions, affecting the complexity and computational requirements of the tensor train.

\subsubsection{Reshaping}
Reshaping in the context of tensor trains involves changing the shape of the tensors without altering the underlying data. This operation can lead to a variation in the bond dimensions if the reshaping process introduces or eliminates dimensions. For example, reshaping a tensor to have more dimensions can increase the length of the tensor train, potentially requiring higher bond dimensions to maintain the same level of accuracy.

\begin{equation}
\text{Reshape:} \quad \mathbf{T} \in \mathbb{R}^{n_1 \times n_2 \times \cdots \times n_d} \rightarrow \mathbf{T'} \in \mathbb{R}^{m_1 \times m_2 \times \cdots \times m_{d'}},
\end{equation}

where the total number of elements remains constant, but the arrangement and possibly the number of bonds change, impacting the bond dimensions $\chi$.

\subsubsection{Slicing}
Slicing refers to the operation of selecting a specific part of the tensor, effectively reducing its dimensionality or size. In tensor trains, slicing can reduce the bond dimensions since it typically involves fixing certain indices, which reduces the complexity of the tensor representation. This operation can significantly decrease the storage and computational requirements by simplifying the tensor structure.

\begin{equation}
\text{Slice:} \quad \mathbf{T}[i_1, :, i_3, :] \rightarrow \mathbf{T'} \in \mathbb{R}^{n_2 \times n_4},
\end{equation}

illustrating how selecting specific indices (fixing $i_1$ and $i_3$) reduces the overall tensor and impacts the associated bond dimensions.

\subsubsection{Contracting}
Tensor contraction is a fundamental operation in tensor networks that combines two tensors into one, summing over a shared index. This operation is closely related to the matrix multiplication in linear algebra but applied within the tensor train context. Contracting tensors can significantly increase the bond dimensions between the contracted tensors, as it combines their information content.

\begin{equation}
\text{Contract:} \quad (\mathbf{T}_1 \times \mathbf{T}_2)_{i_1, \ldots, i_{d-1}, j_1, \ldots, j_{e-1}} = \sum_k \mathbf{T}_1[i_1, \ldots, i_{d-1}, k] \cdot \mathbf{T}_2[k, j_1, \ldots, j_{e-1}],
\end{equation}

where the bond dimension associated with the summation index $k$ dictates the size of the resulting tensor and the complexity of the operation.

\paragraph{Impact on Bond Dimensions}
These basic operations illustrate the dynamic nature of bond dimensions in tensor trains. Reshaping and slicing can reduce the complexity of tensor trains, potentially lowering bond dimensions, while contracting operations can increase bond dimensions due to the integration of information from multiple tensors. Understanding these dynamics is crucial for effectively managing the computational resources and accuracy of tensor train decompositions.

==> sections/introfem.tex <==
\section{Introduction to Finite Element}

\subsection{The Garlekin Method}

The Garlekin method is a technique for finding approximate solutions to differential equations, particularly useful for solving boundary value problems. The method involves selecting a finite-dimensional subspace of the solution space and projecting the residual (error) of the differential equation onto this subspace, ensuring that the residual is orthogonal to the subspace.

\subsubsection{Basic Idea}

Consider a differential equation of the form:
\begin{equation}
Lu = f \quad \text{in} \quad \Omega,
\end{equation}
with boundary conditions:
\begin{equation}
Bu = g \quad \text{on} \quad \partial \Omega,
\end{equation}
where \( L \) is a differential operator, \( \Omega \) is the domain, \( \partial \Omega \) is the boundary of the domain, \( u \) is the unknown solution, \( f \) is a given function, and \( B \) is a boundary operator.

\subsubsection{Weak Formulation}

First, we formulate the weak form of the differential equation. Multiply the differential equation by a test function \( v \) from a suitable function space \( V \) and integrate over the domain \( \Omega \):
\begin{equation}
\int_{\Omega} v (Lu - f) \, d\Omega = 0.
\end{equation}

Applying integration by parts (or Green's theorem) to move derivatives from \( u \) to \( v \) (if \( L \) is a second-order differential operator), we obtain:
\begin{equation}
\int_{\Omega} (L^* v) u \, d\Omega - \int_{\partial \Omega} v (Bu) \, d\Gamma = \int_{\Omega} v f \, d\Omega,
\end{equation}
where \( L^* \) is the adjoint operator of \( L \).

\subsubsection{Approximation}

To approximate the solution \( u \), we choose a finite-dimensional subspace \( V_h \subset V \) and seek an approximate solution \( u_h \in V_h \). The approximate solution can be expressed as:
\begin{equation}
u_h = \sum_{j=1}^n \alpha_j \phi_j,
\end{equation}
where \( \{\phi_j\}_{j=1}^n \) are the basis functions of \( V_h \), and \( \alpha_j \) are the coefficients to be determined.

\subsubsection{Garlekin Condition}

The Garlekin method imposes the condition that the residual is orthogonal to every basis function \( \phi_i \) in \( V_h \):
\begin{equation}
\int_{\Omega} \phi_i (Lu_h - f) \, d\Omega = 0 \quad \forall \, i = 1, \ldots, n.
\end{equation}

Substituting the approximate solution \( u_h \) into this equation gives:
\begin{equation}
\int_{\Omega} \phi_i \left( L \left( \sum_{j=1}^n \alpha_j \phi_j \right) - f \right) \, d\Omega = 0 \quad \forall \, i = 1, \ldots, n.
\end{equation}

\subsubsection{System of Equations}

This leads to a system of linear equations for the coefficients \( \alpha_j \):
\begin{equation}
\sum_{j=1}^n \alpha_j \int_{\Omega} \phi_i L \phi_j \, d\Omega = \int_{\Omega} \phi_i f \, d\Omega \quad \forall \, i = 1, \ldots, n.
\end{equation}

In matrix form, this can be written as:
\begin{equation}
\mathbf{K} \boldsymbol{\alpha} = \mathbf{F},
\end{equation}
where:
\begin{itemize}
    \item \( \mathbf{K} \) is the stiffness matrix with elements \( K_{ij} = \int_{\Omega} \phi_i L \phi_j \, d\Omega \).
    \item \( \boldsymbol{\alpha} \) is the vector of coefficients \( \alpha_j \).
    \item \( \mathbf{F} \) is the load vector with elements \( F_i = \int_{\Omega} \phi_i f \, d\Omega \).
\end{itemize}


\subsection{Finite Element Method (FEM)}

The Finite Element Method (FEM) is a specific implementation of the Garlekin method tailored for solving partial differential equations (PDEs). It involves discretizing the domain into finite elements and using piecewise polynomial basis functions within each element to approximate the solution.

\subsubsection{Domain Discretization}

The first step in FEM is to discretize the domain \( \Omega \) into smaller, non-overlapping subdomains called finite elements. These elements can be of various shapes, such as triangles or quadrilaterals in 2D, and tetrahedra or hexahedra in 3D. The collection of all elements is called the mesh.

\subsubsection{Basis Functions}

Within each finite element, we define a set of local basis functions. These basis functions are typically chosen to be simple polynomials, such as linear or quadratic functions. A common choice for the basis functions is the set of Lagrange polynomials, which are constructed to be 1 at one node and 0 at all other nodes within an element.

Let \( \{ \phi_j \} \) be the set of basis functions associated with the nodes of the elements. The approximate solution \( u_h \) can then be expressed as:
\begin{equation}
u_h = \sum_{j=1}^n \alpha_j \phi_j,
\end{equation}
where \( \alpha_j \) are the coefficients to be determined.

\subsubsection{Weak Formulation and Garlekin Condition}

As in the general Garlekin method, we start with the weak form of the differential equation. Multiply the differential equation by a test function \( v \in V_h \) and integrate over the domain:
\begin{equation}
\int_{\Omega} v (Lu_h - f) \, d\Omega = 0 \quad \forall \, v \in V_h.
\end{equation}

By choosing the test functions \( v \) to be the basis functions \( \phi_i \), we impose the Garlekin condition:
\begin{equation}
\int_{\Omega} \phi_i (Lu_h - f) \, d\Omega = 0 \quad \forall \, i = 1, \ldots, n.
\end{equation}

Substituting the approximate solution \( u_h \) into this equation gives:
\begin{equation}
\int_{\Omega} \phi_i \left( L \left( \sum_{j=1}^n \alpha_j \phi_j \right) - f \right) \, d\Omega = 0 \quad \forall \, i = 1, \ldots, n.
\end{equation}

\subsubsection{System of Equations}

This leads to a system of linear equations for the coefficients \( \alpha_j \):
\begin{equation}
\sum_{j=1}^n \alpha_j \int_{\Omega} \phi_i L \phi_j \, d\Omega = \int_{\Omega} \phi_i f \, d\Omega \quad \forall \, i = 1, \ldots, n.
\end{equation}

In matrix form, this can be written as:
\begin{equation}
\mathbf{K} \boldsymbol{\alpha} = \mathbf{F},
\end{equation}
where:
\begin{itemize}
    \item \( \mathbf{K} \) is the stiffness matrix with elements \( K_{ij} = \int_{\Omega} \phi_i L \phi_j \, d\Omega \).
    \item \( \boldsymbol{\alpha} \) is the vector of coefficients \( \alpha_j \).
    \item \( \mathbf{F} \) is the load vector with elements \( F_i = \int_{\Omega} \phi_i f \, d\Omega \).
\end{itemize}

\subsubsection{Assembly of Global System}

The local stiffness matrices and load vectors from each element are assembled into a global stiffness matrix and a global load vector, taking into account the connectivity of the elements in the mesh. This assembly process involves summing the contributions from all elements and applying appropriate boundary conditions.

\subsubsection{Solution of Algebraic System}

The global system of equations:
\begin{equation}
\mathbf{K} \boldsymbol{\alpha} = \mathbf{F}
\end{equation}
is then solved using numerical techniques such as Gaussian elimination, LU decomposition, or iterative methods to find the coefficients \( \alpha_j \). These coefficients are used to construct the approximate solution \( u_h \) over the entire domain \( \Omega \).

\subsubsection{Post-processing}

The final step involves post-processing the approximate solution \( u_h \) to compute quantities of interest, such as stresses, strains, heat fluxes, or other physical properties. Visualization techniques are also employed to analyze and interpret the results.

\subsection{Isogeometric Analysis (IGA) with Q4 Basis}

Isogeometric Analysis (IGA) is an advanced numerical method that integrates Computer-Aided Design (CAD) and Finite Element Analysis (FEA) by using the same functions for both geometry representation and solution approximation. This method provides higher continuity and accuracy compared to traditional FEM.

\subsubsection{Concept of IGA}

In IGA, Non-Uniform Rational B-Splines (NURBS) or other spline-based functions are used as basis functions for both the geometry and the solution field. This ensures that the exact geometry of the domain is represented, even with a coarse mesh, and allows for smooth and higher-order approximations.

\subsubsection{Q4 Basis Functions}

For simplicity, we consider a Q4 (quadrilateral with 4 nodes) basis, which is commonly used in traditional FEM and adapted here for IGA. Each element is defined by a bilinear mapping from the parametric space to the physical space.

\subsubsection{Parametric Space and Basis Functions}

Consider a parametric space \(\Xi = [0, 1] \times [0, 1]\). The Q4 basis functions \(N_i(\xi, \eta)\) in the parametric space \((\xi, \eta)\) are given by:
\begin{equation}
N_1(\xi, \eta) = (1 - \xi)(1 - \eta),
\end{equation}
\begin{equation}
N_2(\xi, \eta) = \xi (1 - \eta),
\end{equation}
\begin{equation}
N_3(\xi, \eta) = \xi \eta,
\end{equation}
\begin{equation}
N_4(\xi, \eta) = (1 - \xi) \eta.
\end{equation}

These basis functions are bilinear polynomials that interpolate the solution at the four corner nodes of the quadrilateral element.

\subsubsection{Geometry Representation}

The physical coordinates \((x, y)\) of a point inside the element are mapped from the parametric coordinates \((\xi, \eta)\) using the Q4 basis functions:
\begin{equation}
x(\xi, \eta) = \sum_{i=1}^{4} N_i(\xi, \eta) x_i,
\end{equation}
\begin{equation}
y(\xi, \eta) = \sum_{i=1}^{4} N_i(\xi, \eta) y_i,
\end{equation}
where \((x_i, y_i)\) are the physical coordinates of the four corner nodes.

\subsubsection{Approximate Solution}

The approximate solution \(u_h\) within the element can be expressed similarly using the Q4 basis functions:
\begin{equation}
u_h(\xi, \eta) = \sum_{i=1}^{4} N_i(\xi, \eta) u_i,
\end{equation}
where \(u_i\) are the solution values at the four corner nodes.

\subsubsection{Weak Formulation in IGA}

Following the same principles as in FEM, we formulate the weak form of the governing differential equation. For a linear elasticity problem, for example, the weak form is:
\begin{equation}
\int_{\Omega} \sigma(u_h) : \epsilon(v_h) \, d\Omega = \int_{\Omega} f \cdot v_h \, d\Omega + \int_{\partial \Omega} t \cdot v_h \, d\Gamma,
\end{equation}
where \(\sigma\) is the stress tensor, \(\epsilon\) is the strain tensor, \(v_h\) is a test function from the same space as \(u_h\), \(f\) is the body force, and \(t\) is the traction on the boundary \(\partial \Omega\).

\subsubsection{System of Equations}

By applying the Garlekin method with the Q4 basis functions, we obtain a system of equations:
\begin{equation}
\mathbf{K} \boldsymbol{\alpha} = \mathbf{F},
\end{equation}
where:
\begin{itemize}
    \item \( \mathbf{K} \) is the global stiffness matrix assembled from the element stiffness matrices.
    \item \( \boldsymbol{\alpha} \) is the vector of nodal values of the approximate solution.
    \item \( \mathbf{F} \) is the global force vector.
\end{itemize}

\subsubsection{Assembly and Solution}

The element stiffness matrices and force vectors are assembled into global matrices and vectors, considering the continuity and connectivity of the elements in the mesh. The resulting system of equations is solved to find the nodal values of the approximate solution.

\subsubsection{Advantages of IGA}

IGA offers several advantages over traditional FEM:
\begin{itemize}
    \item \textbf{Exact Geometry Representation:} The use of NURBS or other spline-based functions allows for exact representation of the geometry, even with a coarse mesh.
    \item \textbf{Higher Continuity:} IGA provides higher continuity of the solution within and across elements, which is beneficial for problems involving smooth solutions.
    \item \textbf{Efficiency:} The ability to represent complex geometries and achieve higher accuracy with fewer elements can lead to more efficient computations.
\end{itemize}

